The quantum mechanics of Einstein photons and generalized functions

The article consider an interpretation of Majorana equations as a quantum Lorentz covariant equations for the field of Einstein photon. A photon with "deinterlaced" spins (with diagonal Hamiltonian) is considered, its generalized Green function as a functional on finite test functions and its Schr\"{o}dinger equation are constructed. The generalized process corresponding to this Green function is continued to $\sigma$-additive quantum generalized measure on the space dual to the compact subspace of a photon paths in $L_{2}(-\infty,\infty)$. In this case, the filling of whole space by such quantum field instantly occurs in the evolutionary problem. The last part of the article gives the calculation of the "Casimir forces" arising in this field.

==> siunitx_cyr.tex <==
\ProvidesFile{siunitx.cfg}
% Put any \sisetup{} command here too
\sisetup{%
	locale=DE,
	text-series-to-math=true,
	reset-math-version=false,
	reset-text-series=false,
	input-ignore={},
	group-separator={\,},
	input-decimal-markers={.,},
	output-decimal-marker={,},
	group-minimum-digits=5,
	group-digits=integer,
	inter-unit-product=\ensuremath{{}\cdot{}},
	exponent-product=\ensuremath{\cdot},
	range-independent-prefix=false,
	range-units=single,
	per-mode=single-symbol,
%	range-open-phrase=\ensuremath{\text{от~}},
	range-phrase=\ensuremath{\text{\kern 0pt --\kern 0pt}},
	list-independent-prefix=false,
	list-units=single,
	list-final-separator=\ensuremath{\text{ и~}},
	list-pair-separator=\ensuremath{\text{ и~}},
	list-separator={, },
	product-independent-prefix=false,
	product-units=single,
	retain-explicit-decimal-marker=true,
	retain-explicit-plus=true,
	retain-negative-zero=true,
	retain-zero-uncertainty=true,
	multi-part-units=single,
	separate-uncertainty=true,
	separate-uncertainty-units=bracket,
	input-open-uncertainty={(},
	input-close-uncertainty={)},
	output-open-uncertainty={(},
	output-close-uncertainty={)},
	quantity-product={\hspace{0.25em plus 0.1em minus 0.1em}},
	inter-unit-product=\ensuremath{\cdot},
	tight-spacing=true,
	reset-math-version=false,
	text-series-to-math=true,
	text-family-to-math=true,
	tight-spacing=true,
%	table-format=1.3,
	table-alignment-mode=format,
	table-number-alignment=center,
	input-comparators={<=>\approx\ge\geq\geqslant\gg\ggg\le\leq\leqslant\ll\lll\sim\gtrsim\gnsim\lesssim\lnsim\gtrapprox\gnapprox\lessapprox\lnapprox\pm\nm},
}
%%---------------------------------------------------
%% заплатка
%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolCelsius{ \textdegree\text{C} }
%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolDegree{ \textdegree }
%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolArcminute{ \textacute }
%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolArcsecond{ \textacutedbl }
%%---------------------------------------------------

% Основные единицы (SI base units, Table 1)

% Наименование									Символ размерности Русское наименование Французское наименование Английское наименование Русское обозначение Международное обозначение
% Длина												 L									метр								 mètre										metre									 м									 m
% Масса												 M									килограмм						kilogramme							 kilogram								кг									kg
% Время												 T									секунда							seconde									second									с									 s
% Сила электрического тока			I									ампер								ampère									 ampere									А									 A
% Термодинамическая температура Θ									кельвин							kelvin									 kelvin									К									 K
% Количество вещества					 N									моль								 mole										 mole										моль								mol
% Сила света										J									кандела							candela									candela								 кд									cd

\DeclareSIUnit\metre{\text{м}}
\DeclareSIUnit\meter{\text{м}}
%\DeclareSIUnit\kilogram{\text{кг}} % определяется через грамм
\DeclareSIUnit\second{\text{с}}
\DeclareSIUnit\ampere{\text{А}}
\DeclareSIUnit\kelvin{\text{К}}
\DeclareSIUnit\mole{\text{моль}}
\DeclareSIUnit\candela{\text{кд}}


% Производные единицы, имеющие специальные наименования и обозначения (Coherent derived units in the SI with special names and symbols, Table 2)

% Величина																 Русское наименование Английское наименование Русское обозначение Международное обозначение Выражение через основные единицы
% Активность радиоактивного источника			беккерель						becquerel							 Бк									Bq												с−1
% Температура Цельсия											градус Цельсия			 degree Celsius					°C									°C												K
% Электрический заряд											кулон								coulomb								 Кл									C												 А·с
% Электроёмкость													 фарад								farad									 Ф									 F												 Кл/В=с4·А2·кг−1·м−2
% Масса																		грамм								gram										г									 g												 10-3кг
% Поглощённая доза ионизирующего излучения грей								 gray										Гр									Gy												Дж/кг=м²/c²
% Частота																	герц								 hertz									 Гц									Hz												с−1
% Индуктивность														генри								henry									 Гн									H												 кг·м2·с−2·А−2
% Энергия																	джоуль							 joule									 Дж									J												 Н·м=кг·м2·c−2
% Активность катализатора									катал								katal									 кат								 kat											 моль/с
% Световой поток													 люмен								lumen									 лм									lm												кд·ср
% Освещённость														 люкс								 lux										 лк									lx												лм/м²=кд·ср/м²
% Сила																		 ньютон							 newton									Н									 N												 кг·м·c−2
% Сопротивление														ом									 ohm										 Ом									Ω												 В/А=кг·м2·с−3·А−2
% Давление																 паскаль							pascal									Па									Pa												Н/м2=кг·м−1·с−2
% Плоский угол														 радиан							 radian									рад								 rad											 м·м−1=1
% Электрическая проводимость							 сименс							 siemens								 См									S												 Ом−1=с3·А2·кг−1·м−2
% Эффективная доза ионизирующего излучения зиверт							 sievert								 Зв									Sv												Дж/кг=м²/c²
% Телесный угол														стерадиан						steradian							 ср									sr												м2·м−2=1
% Магнитная индукция											 тесла								tesla									 Тл									T												 Вб/м2=кг·с−2·А−1
% Разность потенциалов										 вольт								volt										В									 V												 Дж/Кл=кг·м2·с−3·А−1
% Мощность																 ватт								 watt										Вт									W												 Дж/с=кг·м2·c−3
% Магнитный поток													вебер								weber									 Вб									Wb												кг·м2·с−2·А−1

\DeclareSIUnit\becquerel{\text{Бк}}
%\DeclareSIUnit\degreeCelsius{\text{°C}}
%\DeclareSIUnit\degreeCelsius{ \SIUnitSymbolCelsius }
%%---------------------------------------------------
%\DeclareSIUnit\celsius{ \SIUnitSymbolCelsius }
%\DeclareSIUnit\celsius{{$^{\circ}$C}}	% Nikolaev N.E.
\DeclareSIUnit\dptr{\text{дптр}}	% Nikolaev N.E.%%---------------------------------------------------
\DeclareSIUnit[quantity-product={}]{\degreeCelsius}{\SIUnitSymbolCelsius}
\DeclareSIUnit[quantity-product={}]{\celsius}{\SIUnitSymbolCelsius}
\DeclareSIUnit\dyn{\text{дин}}
\DeclareSIUnit\atm{\text{атм}}
\DeclareSIUnit\at{\text{ат}}
\DeclareSIUnit\erg{\text{эрг}}
\DeclareSIUnit\earthmass{{\text{\itshape M}_{\oplus}}}
\DeclareSIUnit\terramass{{\text{\itshape M}_{\oplus}}}
\DeclareSIUnit\solarmass{{\text{\itshape M}_{\odot}}}
\DeclareSIUnit\solmass{{\text{\itshape M}_{\odot}}}
\DeclareSIUnit\earthradius{{\text{\itshape R}_{\oplus}}}
\DeclareSIUnit\terraradius{{\text{\itshape R}_{\oplus}}}
\DeclareSIUnit\solarradius{{\text{\itshape R}_{\odot}}}
\DeclareSIUnit\solradius{{\text{\itshape R}_{\odot}}}
\DeclareSIUnit\solarluminosity{{\text{\itshape L}_{\odot}}}
\DeclareSIUnit\solluminosity{{\text{\itshape L}_{\odot}}}
\DeclareSIUnit\solarirradiance{{\text{\itshape I}_{\odot}}}
\DeclareSIUnit\sollirradiance{{\text{\itshape I}_{\odot}}}
\DeclareSIUnit\unit{\text{ед.}}
\DeclareSIUnit\units{\text{ед.}}
\DeclareSIUnit\piece{\text{шт.}}
\DeclareSIUnit\pieces{\text{шт.}}
\DeclareSIUnit\item{\text{шт.}}
\DeclareSIUnit\items{\text{шт.}}
\DeclareSIUnit\circulation{\text{экз.}}
\DeclareSIUnit\copies{\text{коп.}}
\DeclareSIUnit[quantity-product={}]\percent{{\%}}
\DeclareSIUnit[quantity-product={}]\procent{{\%}}
\DeclareSIUnit[quantity-product={}]\permille{{$\text{\textperthousand}$}}
\DeclareSIUnit[quantity-product={}]\promille{{$\text{\textperthousand}$}}
\DeclareSIUnit[quantity-product={}]\permyriad{{$\text{\textpertenthousand}$}}
\DeclareSIUnit[quantity-product={}]\promyriad{{$\text{\textpertenthousand}$}}
\DeclareSIUnit\crystalmass{\text{Мк}}
\DeclareSIUnit\absorbance{\text{AU}}
\DeclareSIUnit\opticdensity{\text{D}}
\DeclareSIUnit\Molar{\text{М}}
\DeclareSIUnit\molar{\text{М}}
\DeclareSIUnit\meterwaterequivalent{\text{м в.\,э.}}
\DeclareSIUnit\metrewaterequivalent{\text{м в.\,э.}}
\DeclareSIUnit\mwe{\text{м в.\,э.}}
\DeclareSIUnit\PeV{\peta\eV}
\DeclareSIUnit\EeV{\exa\eV}
\DeclareSIUnit\ZeV{\zetta\eV}
\DeclareSIUnit\YeV{\yotta\eV}
\DeclareSIUnit\mo{\text{мес.}}
\DeclareSIUnit\y{\text{г.}}
\DeclareSIUnit\yr{\text{г.}}
\DeclareSIUnit\yrs{\text{лет}}
\DeclareSIUnit\yyr{\text{гг.}}
\DeclareSIUnit\tropicyear{\ensuremath{\text{a}_{\text{t}}}}
\DeclareSIUnit\julianyear{\ensuremath{\text{a}_{\text{j}}}}
\DeclareSIUnit\gregorianyear{\ensuremath{\text{a}_{\text{g}}}}
\DeclareSIUnit\year{\text{a}}
\DeclareSIUnit\gravaccel{\text{$g$}}
\DeclareSIUnit[qualifier-mode=combine]{\dBm}{\deci\bel\of{\text{м}}}
%%---------------------------------------------------
\DeclareSIUnit\coulomb{\text{Кл}}
\DeclareSIUnit\farad{\text{Ф}}
\DeclareSIUnit\gram{\text{г}}
\DeclareSIUnit\gray{\text{Гр}}
\DeclareSIUnit\hertz{\text{Гц}}
\DeclareSIUnit\henry{\text{Гн}}
\DeclareSIUnit\joule{\text{Дж}}
\DeclareSIUnit\katal{\text{кат}}
\DeclareSIUnit\lumen{\text{лм}}
\DeclareSIUnit\lux{\text{лк}}
\DeclareSIUnit\newton{\text{Н}}
\DeclareSIUnit\ohm{\text{Ом}}
\DeclareSIUnit\pascal{\text{Па}}
\DeclareSIUnit\radian{\text{рад}}
\DeclareSIUnit\siemens{\text{См}}
\DeclareSIUnit\sievert{\text{Зв}}
\DeclareSIUnit\steradian{\text{ср}}
\DeclareSIUnit\tesla{\text{Тл}}
\DeclareSIUnit\volt{\text{В}}
\DeclareSIUnit\watt{\text{Вт}}
\DeclareSIUnit\weber{\text{Вб}}


% Единицы, не входящие в СИ (Non-SI units accepted for use with the International System of Units, Table 3)

% Единица				 Английское наименование Русское обозначение Международное обозначение Величина в единицах СИ
% сутки					 day										 сут								 d												 24ч=86400с
% угловой градус	degree									°									 °												 (π/180)рад
% минута					minute									мин								 min											 60с
% гектар					hectare								 га									ha												10000м²
% час						 hour										ч									 h												 60мин=3600с
% литр						litre									 л									 l,L											 0,001м³
% угловая минута	minute									′									 ′												 (1/60)°=(π/10800)
% угловая секунда second									″									 ″												 (1/60)′=(π/648000)
% тонна					 tonne									 т									 t												 1000кг

\DeclareSIUnit\day{\text{сут}}
%\DeclareSIUnit\degree{\text{°}}
%\DeclareSIUnit[ quantity-product = ]\degree{ \SIUnitSymbolDegree }
\DeclareSIUnit\hectare{\text{га}}
\DeclareSIUnit\hour{\text{ч}}
\DeclareSIUnit\litre{\text{л}}
\DeclareSIUnit\liter{\text{л}}
%\DeclareSIUnit [ quantity-product = ] \arcmin { \arcminute }
%\DeclareSIUnit\arcminute{\text{′}}
%\DeclareSIUnit [ quantity-product = ] \arcminute { \SIUnitSymbolArcminute }
\DeclareSIUnit\minute{\text{мин}}
%\DeclareSIUnit\arcsecond{\text{″}}
%\DeclareSIUnit [ quantity-product = ] \arcsecond { \SIUnitSymbolArcsecond }
\DeclareSIUnit\tonne{\text{т}}


% Non-SI units whose values in SI units must be obtained experimentally, Table 4

\DeclareSIUnit\astronomicalunit{\text{а.е.}}
\DeclareSIUnit\atomicmassunit{\text{а.е.м.}}
\DeclareSIUnit\bohr{ \text { \ensuremath { a_{0} } } }
\DeclareSIUnit\clight{ \text { \ensuremath { c } } }
\DeclareSIUnit\dalton{\text{а.е.м.}}
\DeclareSIUnit\electronmass { \text { \ensuremath { m_{\textup{e}} } } }
\DeclareSIUnit\electronvolt{\text{эВ}}
%\elementarycharge
\DeclareSIUnit\hartree{ \text { \ensuremath { E_{\textup{h}} } } }
\DeclareSIUnit\planckbar{ \text { \ensuremath { \hbar } } }


% Other non-SI units, Table 5

% Единица			Английское наименование Русское обозначение Международное обозначение Величина в единицах СИ
% ангстрем		 ångström								Å									 Å												 10−10м
% бар					bar										 бар								 bar											 100000 Па
% барн				 barn										б									 b												 10−28м²
% бел					bel										 Б									 B												 безразмерна
% узел				 knot										уз									kn												1 морская миля в час = (1852/3600) м/с
% морская миля nautical mile					 миля								M												 1852 м (точно)
% непер				neper									 Нп									Np												безразмерна

\DeclareSIUnit\angstrom{\text{\AA}}
%\DeclareSIUnit\angstrom{\SIUnitSymbolAngstrom}
\DeclareSIUnit\are{\text{а}} % ар (100 м²) не имеет макроса в siunitx по умолчанию
\DeclareSIUnit\bar{\text{бар}}
\DeclareSIUnit\barn{\text{б}}
\DeclareSIUnit\bel{\text{Б}}
\DeclareSIUnit\decibel{\text{дБ}}
\DeclareSIUnit\knot{\text{уз}}
\DeclareSIUnit\mmHg{\text{мм\,рт.ст.}}
\DeclareSIUnit\nauticalmile{\text{миля}}
\DeclareSIUnit\neper{\text{Нп}}


% SI prefixes, Table 6

% Степень Русская приставка Международная приставка Русское обозначение Международное обозначение
% 1			 дека							deca										да									da
% 2			 гекто						 hecto									 г									 h
% 3			 кило							kilo										к									 k
% 6			 мега							mega										М									 M
% 9			 гига							giga										Г									 G
% 12			тера							tera										Т									 T
% 15			пета							peta										П									 P
% 18			экса							exa										 Э									 E
% 21			зетта						 zetta									 З									 Z
% 24			иотта						 yotta									 И									 Y

\DeclareSIPrefix\deca{\text{да}}{1}
\DeclareSIPrefix\hecto{\text{г}}{2}
\DeclareSIPrefix\kilo{\text{к}}{3}
\DeclareSIPrefix\mega{\text{М}}{6}
\DeclareSIPrefix\giga{\text{Г}}{9}
\DeclareSIPrefix\tera{\text{Т}}{12}
\DeclareSIPrefix\peta{\text{П}}{15}
\DeclareSIPrefix\exa{\text{Э}}{18}
\DeclareSIPrefix\zetta{\text{З}}{21}
\DeclareSIPrefix\yotta{\text{И}}{24}


% Степень Русская приставка Международная приставка Русское обозначение Международное обозначение
% -1			деци							deci										д									 d
% -2			санти						 centi									 с									 c
% -3			милли						 milli									 м									 m
% -6			микро						 micro									 мк									µ
% -9			нано							nano										н									 n
% -12		 пико							pico										п									 p
% -15		 фемто						 femto									 ф									 f
% -18		 атто							atto										а									 a
% -21		 зепто						 zepto									 з									 z
% -24		 иокто						 yocto									 и									 y

\DeclareSIPrefix\deci{\text{д}}{-1}
\DeclareSIPrefix\centi{\text{с}}{-2}
\DeclareSIPrefix\milli{\text{м}}{-3}
\DeclareSIPrefix\micro{\text{мк}}{-6}
\DeclareSIPrefix\nano{\text{н}}{-9}
\DeclareSIPrefix\pico{\text{п}}{-12}
\DeclareSIPrefix\femto{\text{ф}}{-15}
\DeclareSIPrefix\atto{\text{а}}{-18}
\DeclareSIPrefix\zepto{\text{з}}{-21}
\DeclareSIPrefix\yocto{\text{и}}{-24}


% Степень Международное обозначение Международная приставка Русское обозначение Русское написание числа бит Русская приставка
% 10			kibi											Ki											киби								Кибит											 Ки
% 20			mebi											Mi											меби								Мибит											 Ми
% 30			gibi											Gi											гиби								Гибит											 Ги
% 40			tebi											Ti											теби								Тибит											 Ти
% 50			pebi											Pi											пеби								Пибит											 Пи
% 60			exbi											Ei											эксби							 Эибит											 Эи
% 70			zebi											Zi											зеби								Зибит											 Зи
% 80			yobi											Yi											йоби								Йибит											 Йи

\DeclareBinaryPrefix\kibi{\text{Ки}}{10}
\DeclareBinaryPrefix\mebi{\text{Ми}}{20}
\DeclareBinaryPrefix\gibi{\text{Ги}}{30}
\DeclareBinaryPrefix\tebi{\text{Ти}}{40}
\DeclareBinaryPrefix\pebi{\text{Пи}}{50}
\DeclareBinaryPrefix\exbi{\text{Эи}}{60}
\DeclareBinaryPrefix\zebi{\text{Зи}}{70}
\DeclareBinaryPrefix\yobi{\text{Йи}}{80}



% Положение о единицах величин, допускаемых к применению в Российской Федерации,
% разрешает применение следующих внесистемных единиц:
% карат
% град (гон)
% световой год
% парсек
% фут
% дюйм
% килограмм-сила на квадратный сантиметр
% миллиметр водяного столба
% метр водяного столба
% техническая атмосфера
% диоптрия
% текс
% гал
% оборот в секунду
% оборот в минуту
% киловатт-час
% вольт-ампер
% вар
% ампер-час
% бит
% байт
% бит в секунду
% байт в секунду
% рентген
% бэр
% рад
% рентген в секунду
% кюри
% стокс
% калория (международная)
% калория термохимическая
% калория 15-градусная
% калория в секунду
% килокалория в час
% гигакалория в час

% Положение разрешает применять единицы относительных и логарифмических величин, такие как:
% процент
% промилле
% миллионная доля
% децибел
% фон
% октава
% декада

% Допускается также применять единицы времени, получившие широкое распространение, например:
% неделя
% месяц
% год
% век
% тысячелетие

% Не применяются с кратными и дольными приставками СИ наименования и обозначения внесистемных единиц:
% массы
% времени
% плоского угла
% длины
% площади
% давления
% оптической силы
% линейной плотности
% скорости
% ускорения
% частоты вращения

\DeclareSIUnit{\KWH}{\text{кВт\ensuremath{\cdot}ч}}
%\DeclareSIUnit\percent {\text{\char 37}}
\DeclareSIUnit\curie		{\text{Ки}}
\DeclareSIUnit\gal			{\text{Гал}}
\DeclareSIUnit\rad			{\text{рад}}
\DeclareSIUnit\rem			{\text{Бэр}}
\DeclareSIUnit\roentgen {\text{Р}}
\DeclareSIUnit\parsec		{\text{пк}}
\DeclareSIUnit\lightyear {\text{св.год}}
\DeclareSIUnit\torr	{\text{торр}}
\DeclareSIUnit\gon		{\text{град}}
\DeclareSIUnit\gauss		 {\text{Гc}}
\DeclareSIUnit\bit	{\text{б}}
\DeclareSIUnit\byte {\text{Б}}
\DeclareSIUnit\numrange {$--$}


==> siunitx_lat.tex <==
\ProvidesFile{siunitx.cfg}
% Put any \sisetup{} command here too
\sisetup{%
	locale=US,
	text-series-to-math=true,
	reset-math-version=false,
	reset-text-series=false,
	input-ignore={},
	group-separator={\,},
	input-decimal-markers={.,},
	output-decimal-marker={.},
	group-minimum-digits=5,
	group-digits=integer,
	inter-unit-product=\ensuremath{{}\cdot{}},
	exponent-product=\ensuremath{\cdot},
	range-independent-prefix=false,
	range-units=single,
	per-mode=single-symbol,
%	range-open-phrase=\ensuremath{\text{from~}},
	range-phrase=\ensuremath{\text{\kern 0pt --\kern 0pt}},
	list-independent-prefix=false,
	list-units=single,
	list-final-separator=\ensuremath{\text{ and~}},
	list-pair-separator=\ensuremath{\text{ and~}},
	list-separator={, },
	product-independent-prefix=false,
	product-units=single,
	retain-explicit-decimal-marker=true,
	retain-explicit-plus=true,
	retain-negative-zero=true,
	retain-zero-uncertainty=true,
	multi-part-units=single,
	separate-uncertainty=true,
	separate-uncertainty-units=bracket,
	input-open-uncertainty={(},
	input-close-uncertainty={)},
	output-open-uncertainty={(},
	output-close-uncertainty={)},
	quantity-product={\hspace{0.25em plus 0.1em minus 0.1em}},
	inter-unit-product=\ensuremath{\cdot},
	tight-spacing=true,
	reset-math-version=false,
	text-series-to-math=true,
	text-family-to-math=true,
	tight-spacing=true,
%	table-format=1.3,
	table-alignment-mode=format,
	table-number-alignment=center,
	input-comparators={<=>\approx\ge\geq\geqslant\gg\ggg\le\leq\leqslant\ll\lll\sim\gtrsim\gnsim\lesssim\lnsim\gtrapprox\gnapprox\lessapprox\lnapprox\pm\mp},
}
%%%%%---------------------------------------------------
%%%%% заплатка
%%%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolCelsius{ \textdegree\text{C} }
%%%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolDegree{ \textdegree }
%%%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolArcminute{ \textacute }
%%%\DeclareSIUnit[ quantity-product = ]\SIUnitSymbolArcsecond{ \textacutedbl }
%%%%%---------------------------------------------------
%%%
%%%% Основные единицы (SI base units, Table 1)
%%%
%%%% Наименование									Символ размерности Русское наименование Французское наименование Английское наименование Русское обозначение Международное обозначение
%%%% Длина												 L									метр								 mètre										metre									 м									 m
%%%% Масса												 M									килограмм						kilogramme							 kilogram								кг									kg
%%%% Время												 T									секунда							seconde									second									с									 s
%%%% Сила электрического тока			I									ампер								ampère									 ampere									А									 A
%%%% Термодинамическая температура Θ									кельвин							kelvin									 kelvin									К									 K
%%%% Количество вещества					 N									моль								 mole										 mole										моль								mol
%%%% Сила света										J									кандела							candela									candela								 кд									cd
%%%
\DeclareSIUnit\metre{\text{m}}
\DeclareSIUnit\meter{\text{m}}
%%%%\DeclareSIUnit\kilogram{\text{kg}} % определяется через грамм
\DeclareSIUnit\second{\text{s}}
\DeclareSIUnit\ampere{\text{A}}
\DeclareSIUnit\kelvin{\text{K}}
\DeclareSIUnit\mole{\text{mol}}
\DeclareSIUnit\candela{\text{cd}}
%%%
%%%
%%%% Производные единицы, имеющие специальные наименования и обозначения (Coherent derived units in the SI with special names and symbols, Table 2)
%%%
%%%% Величина																 Русское наименование Английское наименование Русское обозначение Международное обозначение Выражение через основные единицы
%%%% Активность радиоактивного источника			беккерель						becquerel							 Бк									Bq												с−1
%%%% Температура Цельсия											градус Цельсия			 degree Celsius					°C									°C												K
%%%% Электрический заряд											кулон								coulomb								 Кл									C												 А·с
%%%% Электроёмкость													 фарад								farad									 Ф									 F												 Кл/В=с4·А2·кг−1·м−2
%%%% Масса																		грамм								gram										г									 g												 10-3кг
%%%% Поглощённая доза ионизирующего излучения грей								 gray										Гр									Gy												Дж/кг=м²/c²
%%%% Частота																	герц								 hertz									 Гц									Hz												с−1
%%%% Индуктивность														генри								henry									 Гн									H												 кг·м2·с−2·А−2
%%%% Энергия																	джоуль							 joule									 Дж									J												 Н·м=кг·м2·c−2
%%%% Активность катализатора									катал								katal									 кат								 kat											 моль/с
%%%% Световой поток													 люмен								lumen									 лм									lm												кд·ср
%%%% Освещённость														 люкс								 lux										 лк									lx												лм/м²=кд·ср/м²
%%%% Сила																		 ньютон							 newton									Н									 N												 кг·м·c−2
%%%% Сопротивление														ом									 ohm										 Ом									Ω												 В/А=кг·м2·с−3·А−2
%%%% Давление																 паскаль							pascal									Па									Pa												Н/м2=кг·м−1·с−2
%%%% Плоский угол														 радиан							 radian									рад								 rad											 м·м−1=1
%%%% Электрическая проводимость							 сименс							 siemens								 См									S												 Ом−1=с3·А2·кг−1·м−2
%%%% Эффективная доза ионизирующего излучения зиверт							 sievert								 Зв									Sv												Дж/кг=м²/c²
%%%% Телесный угол														стерадиан						steradian							 ср									sr												м2·м−2=1
%%%% Магнитная индукция											 тесла								tesla									 Тл									T												 Вб/м2=кг·с−2·А−1
%%%% Разность потенциалов										 вольт								volt										В									 V												 Дж/Кл=кг·м2·с−3·А−1
%%%% Мощность																 ватт								 watt										Вт									W												 Дж/с=кг·м2·c−3
%%%% Магнитный поток													вебер								weber									 Вб									Wb												кг·м2·с−2·А−1
%%%
\DeclareSIUnit\becquerel{\text{Bq}}
%%%%\DeclareSIUnit\degreeCelsius{\text{°C}}
%\DeclareSIUnit\degreeCelsius{ \SIUnitSymbolCelsius }
%%%%%---------------------------------------------------
%%%%\DeclareSIUnit\celsius{ \SIUnitSymbolCelsius }
%\DeclareSIUnit\celsius{{$^{\circ}$C}}	% Nikolaev N.E.
\DeclareSIUnit\dptr{\text{dpt}}	% Nikolaev N.E.
%%%%%---------------------------------------------------
\DeclareSIUnit[quantity-product={}]{\degreeCelsius}{\SIUnitSymbolCelsius}
\DeclareSIUnit[quantity-product={}]{\celsius}{\SIUnitSymbolCelsius}
\DeclareSIUnit\dyn{\text{dyn}}
\DeclareSIUnit\atm{\text{atm}}
\DeclareSIUnit\at{\text{at}}
\DeclareSIUnit\erg{\text{erg}}
\DeclareSIUnit\earthmass{{\text{\itshape M}_{\oplus}}}
\DeclareSIUnit\terramass{{\text{\itshape M}_{\oplus}}}
\DeclareSIUnit\solarmass{{\text{\itshape M}_{\odot}}}
\DeclareSIUnit\solmass{{\text{\itshape M}_{\odot}}}
\DeclareSIUnit\earthradius{{\text{\itshape R}_{\oplus}}}
\DeclareSIUnit\terraradius{{\text{\itshape R}_{\oplus}}}
\DeclareSIUnit\solarradius{{\text{\itshape R}_{\odot}}}
\DeclareSIUnit\solradius{{\text{\itshape R}_{\odot}}}
\DeclareSIUnit\solarluminosity{{\text{\itshape L}_{\odot}}}
\DeclareSIUnit\solluminosity{{\text{\itshape L}_{\odot}}}
\DeclareSIUnit\solarirradiance{{\text{\itshape I}_{\odot}}}
\DeclareSIUnit\sollirradiance{{\text{\itshape I}_{\odot}}}
\DeclareSIUnit\unit{\text{unit}}
\DeclareSIUnit\units{\text{units}}
\DeclareSIUnit\piece{\text{pce}}
\DeclareSIUnit\pieces{\text{pcs}}
\DeclareSIUnit\item{\text{item}}
\DeclareSIUnit\items{\text{items}}
\DeclareSIUnit\circulation{\text{cop.}}
\DeclareSIUnit\copies{\text{cop.}}
\DeclareSIUnit[quantity-product={}]{\percent}{{\%}}
\DeclareSIUnit[quantity-product={}]{\procent}{{\%}}
\DeclareSIUnit[quantity-product={}]{\permille}{{$\text{\textperthousand}$}}
\DeclareSIUnit[quantity-product={}]{\promille}{{$\text{\textperthousand}$}}
\DeclareSIUnit[quantity-product={}]{\permyriad}{{$\text{\textpertenthousand}$}}
\DeclareSIUnit[quantity-product={}]{\promyriad}{{$\text{\textpertenthousand}$}}
\DeclareSIUnit\crystalmass{\text{Mc}}
\DeclareSIUnit\absorbance{\text{AU}}
\DeclareSIUnit\opticdensity{\text{D}}
\DeclareSIUnit\Molar{\text{M}}
\DeclareSIUnit\molar{\text{M}}
\DeclareSIUnit\meterwaterequivalent{\text{m.w.e.}}
\DeclareSIUnit\metrewaterequivalent{\text{m.w.e.}}
\DeclareSIUnit\mwe{\text{m.w.e.}}
\DeclareSIUnit\PeV{\peta\eV}
\DeclareSIUnit\EeV{\exa\eV}
\DeclareSIUnit\ZeV{\zetta\eV}
\DeclareSIUnit\YeV{\yotta\eV}
\DeclareSIUnit\mo{\text{mo}}
\DeclareSIUnit\y{\text{y}}
\DeclareSIUnit\yr{\text{yr}}
\DeclareSIUnit\yrs{\text{yr}}
\DeclareSIUnit\yyr{}
\DeclareSIUnit\tropicyear{\ensuremath{\text{a}_{\text{t}}}}
\DeclareSIUnit\julianyear{\ensuremath{\text{a}_{\text{j}}}}
\DeclareSIUnit\gregorianyear{\ensuremath{\text{a}_{\text{g}}}}
\DeclareSIUnit\year{\text{a}}
\DeclareSIUnit\gravaccel{\text{$g$}}
\DeclareSIUnit[qualifier-mode=combine]{\dBm}{\deci\bel\of{m}}
%%%%%---------------------------------------------------
\DeclareSIUnit\coulomb{\text{C}}
\DeclareSIUnit\farad{\text{F}}
\DeclareSIUnit\gram{\text{g}}
\DeclareSIUnit\gray{\text{Gy}}
\DeclareSIUnit\hertz{\text{Hz}}
\DeclareSIUnit\henry{\text{H}}
\DeclareSIUnit\joule{\text{J}}
\DeclareSIUnit\katal{\text{kat}}
\DeclareSIUnit\lumen{\text{lm}}
\DeclareSIUnit\lux{\text{lx}}
\DeclareSIUnit\newton{\text{N}}
\DeclareSIUnit\ohm{\text{\Omega}}
\DeclareSIUnit\pascal{\text{Pa}}
\DeclareSIUnit\radian{\text{rad}}
\DeclareSIUnit\siemens{\text{S}}
\DeclareSIUnit\sievert{\text{Sv}}
\DeclareSIUnit\steradian{\text{sr}}
\DeclareSIUnit\tesla{\text{T}}
\DeclareSIUnit\volt{\text{V}}
\DeclareSIUnit\watt{\text{W}}
\DeclareSIUnit\weber{\text{Wb}}
%%%
%%%
%%%% Единицы, не входящие в СИ (Non-SI units accepted for use with the International System of Units, Table 3)
%%%
%%%% Единица				 Английское наименование Русское обозначение Международное обозначение Величина в единицах СИ
%%%% сутки					 day										 сут								 d												 24ч=86400с
%%%% угловой градус	degree									°									 °												 (π/180)рад
%%%% минута					minute									мин								 min											 60с
%%%% гектар					hectare								 га									ha												10000м²
%%%% час						 hour										ч									 h												 60мин=3600с
%%%% литр						litre									 л									 l,L											 0,001м³
%%%% угловая минута	minute									′									 ′												 (1/60)°=(π/10800)
%%%% угловая секунда second									″									 ″												 (1/60)′=(π/648000)
%%%% тонна					 tonne									 т									 t												 1000кг
%%%
\DeclareSIUnit\day{\text{d}}
%\DeclareSIUnit\degree{\text{°}}
%\DeclareSIUnit[ quantity-product = ]\degree{ \SIUnitSymbolDegree }
\DeclareSIUnit\hectare{\text{ha}}
\DeclareSIUnit\hour{\text{h}}
\DeclareSIUnit\litre{\text{L}}
\DeclareSIUnit\liter{\text{L}}
\DeclareSIUnit [ quantity-product = ] \arcmin { \arcminute }
%\DeclareSIUnit\arcminute{\text{′}}
\DeclareSIUnit [ quantity-product = ] \arcminute { \SIUnitSymbolArcminute }
\DeclareSIUnit\minute{\text{min}}
%\DeclareSIUnit\arcsecond{\text{″}}
\DeclareSIUnit [ quantity-product = ] \arcsecond { \SIUnitSymbolArcsecond }
\DeclareSIUnit\tonne{\text{t}}
%%%
%%%
%%%% Non-SI units whose values in SI units must be obtained experimentally, Table 4
%%%
\DeclareSIUnit\astronomicalunit{\text{au}}
\DeclareSIUnit\atomicmassunit{\text{Da}}
\DeclareSIUnit\bohr{ \text { \ensuremath { a_{0} } } }
\DeclareSIUnit\clight{ \text { \ensuremath { c } } }
\DeclareSIUnit\dalton{\text{Da}}
\DeclareSIUnit\electronmass { \text { \ensuremath { m_{\textup{e}} } } }
\DeclareSIUnit\electronvolt{\text{eV}}
%\elementarycharge
\DeclareSIUnit\hartree{ \text { \ensuremath { E_{\textup{h}} } } }
\DeclareSIUnit\planckbar{ \text { \ensuremath { \hbar } } }
%%%
%%%
%%%% Other non-SI units, Table 5
%%%
%%%% Единица			Английское наименование Русское обозначение Международное обозначение Величина в единицах СИ
%%%% ангстрем		 ångström								Å									 Å												 10−10м
%%%% бар					bar										 бар								 bar											 100000 Па
%%%% барн				 barn										б									 b												 10−28м²
%%%% бел					bel										 Б									 B												 безразмерна
%%%% узел				 knot										уз									kn												1 морская миля в час = (1852/3600) м/с
%%%% морская миля nautical mile					 миля								M												 1852 м (точно)
%%%% непер				neper									 Нп									Np												безразмерна
%%%
\DeclareSIUnit\angstrom{\text{\AA}}
%%%%\DeclareSIUnit\angstrom{\SIUnitSymbolAngstrom}
%%%\DeclareSIUnit\are{\text{а}} % ар (100 м²) не имеет макроса в siunitx по умолчанию
\DeclareSIUnit\bar{\text{bar}}
\DeclareSIUnit\barn{\text{b}}
\DeclareSIUnit\bel{\text{B}}
\DeclareSIUnit\decibel{\text{dB}}
\DeclareSIUnit\knot{\text{knot}}
\DeclareSIUnit\mmHg{\text{mmHg}}
\DeclareSIUnit\nauticalmile{\text{M}}
\DeclareSIUnit\neper{\text{Np}}
%%%
%%%
%%%% SI prefixes, Table 6
%%%
%%%% Степень Русская приставка Международная приставка Русское обозначение Международное обозначение
%%%% 1			 дека							deca										да									da
%%%% 2			 гекто						 hecto									 г									 h
%%%% 3			 кило							kilo										к									 k
%%%% 6			 мега							mega										М									 M
%%%% 9			 гига							giga										Г									 G
%%%% 12			тера							tera										Т									 T
%%%% 15			пета							peta										П									 P
%%%% 18			экса							exa										 Э									 E
%%%% 21			зетта						 zetta									 З									 Z
%%%% 24			иотта						 yotta									 И									 Y
%%%
\DeclareSIPrefix\deca{\text{da}}{1}
\DeclareSIPrefix\hecto{\text{h}}{2}
\DeclareSIPrefix\kilo{\text{k}}{3}
\DeclareSIPrefix\mega{\text{M}}{6}
\DeclareSIPrefix\giga{\text{G}}{9}
\DeclareSIPrefix\tera{\text{T}}{12}
\DeclareSIPrefix\peta{\text{P}}{15}
\DeclareSIPrefix\exa{\text{E}}{18}
\DeclareSIPrefix\zetta{\text{Z}}{21}
\DeclareSIPrefix\yotta{\text{Y}}{24}
%%%
%%%
%%%% Степень Русская приставка Международная приставка Русское обозначение Международное обозначение
%%%% -1			деци							deci										д									 d
%%%% -2			санти						 centi									 с									 c
%%%% -3			милли						 milli									 м									 m
%%%% -6			микро						 micro									 мк									µ
%%%% -9			нано							nano										н									 n
%%%% -12		 пико							pico										п									 p
%%%% -15		 фемто						 femto									 ф									 f
%%%% -18		 атто							atto										а									 a
%%%% -21		 зепто						 zepto									 з									 z
%%%% -24		 иокто						 yocto									 и									 y
%%%
\DeclareSIPrefix\deci{\text{d}}{-1}
\DeclareSIPrefix\centi{\text{c}}{-2}
\DeclareSIPrefix\milli{\text{m}}{-3}
\DeclareSIPrefix\micro{\text{\mu}}{-6}
\DeclareSIPrefix\nano{\text{n}}{-9}
\DeclareSIPrefix\pico{\text{p}}{-12}
\DeclareSIPrefix\femto{\text{f}}{-15}
\DeclareSIPrefix\atto{\text{a}}{-18}
\DeclareSIPrefix\zepto{\text{z}}{-21}
\DeclareSIPrefix\yocto{\text{y}}{-24}
%%%
%%%
%%%% Степень Международное обозначение Международная приставка Русское обозначение Русское написание числа бит Русская приставка
%%%% 10			kibi											Ki											киби								Кибит											 Ки
%%%% 20			mebi											Mi											меби								Мибит											 Ми
%%%% 30			gibi											Gi											гиби								Гибит											 Ги
%%%% 40			tebi											Ti											теби								Тибит											 Ти
%%%% 50			pebi											Pi											пеби								Пибит											 Пи
%%%% 60			exbi											Ei											эксби							 Эибит											 Эи
%%%% 70			zebi											Zi											зеби								Зибит											 Зи
%%%% 80			yobi											Yi											йоби								Йибит											 Йи
%%%
\DeclareBinaryPrefix\kibi{\text{Ki}}{10}
\DeclareBinaryPrefix\mebi{\text{Mi}}{20}
\DeclareBinaryPrefix\gibi{\text{Gi}}{30}
\DeclareBinaryPrefix\tebi{\text{Ti}}{40}
\DeclareBinaryPrefix\pebi{\text{Pi}}{50}
\DeclareBinaryPrefix\exbi{\text{Ei}}{60}
\DeclareBinaryPrefix\zebi{\text{Zi}}{70}
\DeclareBinaryPrefix\yobi{\text{Yi}}{80}
%%%
%%%
%%%
%%%% Положение о единицах величин, допускаемых к применению в Российской Федерации,
%%%% разрешает применение следующих внесистемных единиц:
%%%% карат
%%%% град (гон)
%%%% световой год
%%%% парсек
%%%% фут
%%%% дюйм
%%%% килограмм-сила на квадратный сантиметр
%%%% миллиметр водяного столба
%%%% метр водяного столба
%%%% техническая атмосфера
%%%% диоптрия
%%%% текс
%%%% гал
%%%% оборот в секунду
%%%% оборот в минуту
%%%% киловатт-час
%%%% вольт-ампер
%%%% вар
%%%% ампер-час
%%%% бит
%%%% байт
%%%% бит в секунду
%%%% байт в секунду
%%%% рентген
%%%% бэр
%%%% рад
%%%% рентген в секунду
%%%% кюри
%%%% стокс
%%%% калория (международная)
%%%% калория термохимическая
%%%% калория 15-градусная
%%%% калория в секунду
%%%% килокалория в час
%%%% гигакалория в час
%%%
%%%% Положение разрешает применять единицы относительных и логарифмических величин, такие как:
%%%% процент
%%%% промилле
%%%% миллионная доля
%%%% децибел
%%%% фон
%%%% октава
%%%% декада
%%%
%%%% Допускается также применять единицы времени, получившие широкое распространение, например:
%%%% неделя
%%%% месяц
%%%% год
%%%% век
%%%% тысячелетие
%%%
%%%% Не применяются с кратными и дольными приставками СИ наименования и обозначения внесистемных единиц:
%%%% массы
%%%% времени
%%%% плоского угла
%%%% длины
%%%% площади
%%%% давления
%%%% оптической силы
%%%% линейной плотности
%%%% скорости
%%%% ускорения
%%%% частоты вращения
%%%
\DeclareSIUnit{\KWH}{\text{kW\ensuremath{\cdot}h}}
%\DeclareSIUnit\percent {\text{\char 37}}
\DeclareSIUnit\curie		{\text{Ci}}
\DeclareSIUnit\gal			{\text{Gal}}
\DeclareSIUnit\rad			{\text{rad}}
\DeclareSIUnit\rem			{\text{rem}}
\DeclareSIUnit\roentgen {\text{R}}
\DeclareSIUnit\parsec		{\text{pc}}
\DeclareSIUnit\lightyear {\text{ly}}
\DeclareSIUnit\torr	{\text{Torr}}
\DeclareSIUnit\gon		{\text{gon}}
\DeclareSIUnit[ quantity-product = ]\arcgon{ $^{\text{g}}$ }
\DeclareSIUnit\gauss		 {\text{G}}
\DeclareSIUnit\bit	{\text{b}}
\DeclareSIUnit\byte {\text{B}}
\DeclareSIUnit\numrange {$--$}

